Fermi Large Area Telescope Performance After 10 Years Of Operation

The Large Area Telescope (LAT), the primary instrument for the Fermi Gamma-ray Space Telescope (Fermi) mission, is an imaging, wide field-of-view, high-energy gamma-ray telescope, covering the energy range from 30 MeV to more than 300 GeV. We describe the performance of the instrument at the 10-year milestone. LAT performance remains well within the specifications defined during the planning phase, validating the design choices and supporting the compelling case to extend the duration of the Fermi mission. The details provided here will be useful when designing the next generation of high-energy gamma-ray observatories.

==> cal_failures.tex <==
\subsection{Calorimeter component failures}

One preamplifier out of 6144 failed. Signal disappeared in 2010 July, with no change in noise, noise started misbehaving on 2017 August, enough to fire the L0 trigger request. Disabled automatic range selection and L0 request for the corresponding front-end ASIC.                                                                                                                                                  

==> oth_summary.tex <==
\subsection{Trending}

Trending of \Fermi\ spacecraft and instrument performance and associated ground operations performance is done continuously. Review and assessment of spacecraft and instrument performance and operations trends is done at weekly intervals in meetings of the spacecraft and instrument operations support teams, and also more comprehensively reviewed and assessed at 3-month intervals. Performance is trended within the reporting period, and also over the mission lifetime.

Both direct and derived measurements are trended, for both spacecraft and instruments.

Some key performance parameters that are trended for the spacecraft and mission, and that are most relevant to the LAT, are:
\begin{itemize}
    \item orbit altitude
    \item use of on-board data storage
    \item number of ground contact periods
    \item required time for data down-link
    \item down-linked data recovery percentage
\end{itemize}

Some key performance parameters that are trended for the LAT are:
\begin{itemize}
    \item power supply voltages
    \item power supply currents
    \item temperatures
    \item LAT active thermal control duty cycle
    \item CPU memory errors
    \item number of event triggers on the LAT
    \item LAT fractional up-time for science data-taking
    \item data latency (time interval between raw data being collected on the LAT, and resultant processed and filtered gamma-ray photons being delivered to NASA for public release through the FSSC)
    \item detector calibrations, for each of the Tracker, Calorimeter and ACD detector sub-systems
    \item volume of data stored on the ground
    \item number of gamma-ray events and photons released to the public through the FSSC
\end{itemize}


==> tkr_calib_simo.tex <==
\subsection{Tracker calibration}\label{subsec:tkr_calib}
Detailed descriptions of the calibrated quantities and calibration procedure for the TKR are given in \citet{REF:2009.OnOrbitCalib}.  Here we provide a brief review of the calibration constants and discuss how some of the values have evolved during the mission.


The split point in the front-end daisy chain, nominally splitting the 24 ASICs $12/12$ towards the two controllers, can be electronically moved e.g. to isolate a faulty front end. Before launch, a single frontend ASIC failed, in Tower 10, on Silicon Layer 0. To accommodate this single failed Tracker ASIC, for this single layer, the left/right split has been moved so that all working frontends on this single plane can be read. In orbit, no such other case has occurred, so all other split points are still at their default location of the middle of the plane. 
%\FIXME{RR: Not moved right to that ASIC to collect left and right of it?}



 One overall energy-scale constant allows to convert the electronic signal in any TKR channel into deposited charge and, on top of that, one scale factor per channel allows to tune the energy scale channel by channel. The time evolution of the global energy scale is monitored by observing the energy deposited by minimum-ionizing particles. Some variation is observed in the first months ($\sim 10$\% increase): in \Figref{tkrchscale} the location of the MIP peak before applying this calibration is shown. This is interpreted as initial radiation damage quickly coming to saturation. 
 %\FIXME{After *** no further updates were necessary}. 
 Since this affects directly the energy measurement as a multiplicative constant, good accuracy is necessary. 
 %; \FIXME{2 words about measurement uncertainty, how many \%? Measurements with MIP peak are at low energy, where TKR Emeas is most important, any other comment?}. 
 No channel-by-channel variations above a couple percent are observed, with no significant time evolution.

\twopanel{htb!}{tkrMIPpeak.pdf}{tkrMIPpeak-zoom.pdf}{
  \caption{Trending of the MIP peak energy value during the mission (left) and a zoom of the first weeks after launch (right).}
  \label{fig:tkrchscale}
}


The performances of the individual tracker channels are continuously monitored using both the nominal science data and dedicated calibration runs.
The noise of each channel can be evaluated in calibration runs using the tracker charge injection system, by means of a charge scan  (from 0.8 to 2.6 fC) fixing the discriminators threshold at their nominal value. The resulting ``s-curve'' (add figure????) is fitted to an error function, from which the effective threshold end the equivalent noise charge (ENC) are obtained. 
In figure~\figref{tkrnoisedist}, left, the noise distribution for all the tracker channels  shown for two charge injection runs, one after the launch and one after almost 10 years of mission.The uncertainty on the measurement of the noise level for a single channel is $\sim 7$\%.
Taking the ratio of the values in the later run over the older gives the distribution shown in \figref{tkrnoisedist}, right: the small trend towards values greater than 1 (i.e. increasing noise) is small but visible. In \figref{tkrnoise}, left, the readout noise is averaged over all channels. The relative increase is within expectations (a couple of percent). For comparison in \figref{tkrnoise}, right, the long-term increase of bias current for each TKR module and their total are shown: the noise increase can be correlated with the overall increase in leakage current, attributed to radiation damage. The rapid variations on top of the slowly growing trend in the plot can be correlated to temperature variations, as measured by the sensors in the TKR, in \figref{tkrtemperature}. 

\twopanel{htb!}{tkrnoiseDist}{tkrnoiseRatio}{
  \caption{Tracker noise distribution (a) and ratio (b).}
  \label{fig:tkrnoisedist}
}


\twopanel{htb!}{tkrnoiseTrend_2}{tkrbiasCurrent_2}{
  \caption{Trending of tracker noise (a). For reference, tracker bias current (b).}
  \label{fig:tkrnoise}
}

\begin{figure}[htbp]
  \centering
   \includegraphics[width=\onecolfigwidth]{tkrtemperature_2}
  
  \caption{Temperature, average (black) and each thermistor (gray).}
  \label{fig:tkrtemperature}
\end{figure}


The ENC distribution obtained from charge injection scan allows to identify defective channels: while ``normal'' channels have a typical noise level of $\approx$1300 electrons (mainly determined by
the 1~pF input capacitance of the silicon strip),  channels where the silicon strip is effectively disconnected from the preamplifier input form the  peak at a typical noise of
200 electrons and  dead channels (dead preamplifier) give the single spike at 0. There is also a population of partially disconnected channels, i.e. silicon strips with defective wire bonds along the ladder, that are therefore insensitive in 1/4, 1/2 or 3/4  of the active area, leading to intermediate noise levels.

Since calibration runs reduce the overall LAT livetime, also nominal science data are used to monitor the tracker.  
Noisy channels are a identified (and masked) looking at the strip occupancy (as detailed in  \citet{REF:2009.OnOrbitCalib} ).
The time evolution of bad strips is shown in  \Figref{tkrbadstrips}.
At the time of launch, 3661 readout strips were declared bad (0.31\% of the total); almost 40\% of these were located in Tower 0, the first tower to be assembled.  2047 were strips being disconnected from the readouts,  while 413 channels had a dead preamplifier, and  998 were  partially disconnected strips.  Finally, 203 strips were electronically disabled, being too noisy (0.02\% of total). 
After 10 years of operation in orbit, the number of bad strips increased to 4087 (0.46\%). Surprisingly, the number of disconnected and dead channels diminished to 2008 and 405, respectively,
indicating that in some cases the true cause of the malfunction is not clear and can recover in time. The number of partially disconnected strips increased to 1076, while the number of noisy channels increased to 598 (0.07\%), mostly in Towers 0 and 3. 
In Tower 0, most of the noisy strips are in one ladder on silicon layer 14, and were either noisy before launch or became noisy in the first few weeks after launch. In Tower 3, most of the noisy strips are in one ladder on silicon layer 35 at the top of the tower, nearest the ACD shell. In Tower 3, the noisy ladder started becoming noisy in 2010, and more strips in that ladder became noisy over a period of several years. After 10 years, 58\% of the 598 masked noisy strips were on 2 of the 2304 silicon strip ladders in the LAT.
The recovery from the extended LAT power off period in April 2018 provided more evidence of non-standard behavior of the noisy Si ladder in tower 3. \Figref{TKRbiascurrent2018} shows the TKR bias currents for the 16 towers after the March 2018 LAT power off period. The bias current for tower 3 (the top blue curve) shows a slower recovery over a duration of many days compared to the other towers, as the noise in layer 35 of tower 3 slowly recovered to pre-fault levels over that extended time period. The March 2018 power outage of the LAT did not result in any damage to the TKR subsystem.

\begin{figure}[htbp]
  \centering
    \includegraphics[width=12cm]{tkrbadStrips_2}
  \caption{Dead and noisy channels in the tracker as a function of time.}
  \label{fig:tkrbadstrips}
\end{figure}

\begin{figure}[htbp]
  \centering

  \includegraphics[width=12cm]{figures/biasIrestart_wOfset3.png}
  \caption{Tracker bias currents for the tracker towers after the Fermi safemode and LAT power off period in March 2018. The bias current for tower 3 (the top blue curve) shows a slower recovery over a duration of many days compared to the other towers, as the noise in layer 35 of tower 3 slowly recovered to pre-fault levels over that extended time period.} 
  \label{fig:TKRbiascurrent2018}
\end{figure}

The TKR hit efficiency can be estimated by looking at tracks and counting how often a detected particle passes an active volume without registering a hit, see \figref{tkrefficiencies}, left. The sensitivity of this measurement is $\leq 10^{-4}$, and by interpolating with an exponential?, a decrease in efficiency of $3\cdot 10^{-5}$ per year is apparent, with no practical consequences. Similarly, by looking at how many recorded tracks that should have produced a trigger failed to issue one, we can estimate the TKR trigger efficiency, see \figref{tkrefficiencies}, right. The sensitivity for this estimate is $\sim 10^{-4}$, and an exponential fit gives an increase of trigger efficiency of $2\cdot 10^{-5}$ per year, mostly thanks to a small increase in the first year. 
%\FIXME{I picked the numbers from the pics, someone please check. Also, the trig eff rise seems not statistically significant, can we have errors on these fits?} 
It must be remarked that the exact values in \figref{tkrefficiencies} are also affected by the details of the reconstruction process: notably with the passage to the \peight\ reconstruction a systematic shift of $\pm 0.1$~\% is scaled away from the data, being not relevant for the monitoring of the performance.

\twopanel{htb!}{tkrHitEff.pdf}{tkrTrigEff.pdf}{
  \caption{Tracker hit efficiency (left) and trigger efficiency (right). \peight\ data are scaled for trending purposes. }
  \label{fig:tkrefficiencies}
}

One rotation matrix allows to translate the reconstructed primary direction from TKR to spacecraft (and thence celestial) reference system and, on top of that, translation and rotation offsets of each Si plane in the TKR reference system are accounted for by additional calibration constants.
%Relevant quantities are constantly monitored, and  calibration constants are updated as needed. \FIXME{RR: remove this paragraph?}
The relative alignment of the LAT reference system in the spacecraft reference system, the latter corresponding to the Navigation system and determined by the star-tracker observations, is determined by minimizing the residuals of the measured locations of known \gammaRayHyph\ sources in the sky. The relative alignment is known with an accuracy better than 5~arcsec on the three rotation angles, and show no significant evolution in time.
The relative alignment of each silicon plane in a tower with respect to the LAT reference system is given as 3 offset translations and 3 rotation angles. The sensitivity of the measurement is of $< 1\mu$m ($<2 \mu$m) for the x, y (z) translations, and of $\leq 0.02$~mrad ($\leq 0.01$~mrad) for rotations around the x, y (z) axes. No significant evolution in time is observed. Alignment impacts on the PSF: translation uncertainties are well below the position resolution of a charge cluster (***~$\mu$m), and we estimate that spurious rotations should be $\sim 0.3$~mrad {\em at the tower level} before affecting the high-energy PSF. 
%\FIXME{right? The estimate on the PSF is old, pass6 age, any recent estimate?}. 
In \figref{tkralignment} the calibration constants for each Silicon plane are shown as a function of time, no evolution can be observed.

\begin{figure}[htbp]
  \centering
  \includegraphics[width=0.45\textwidth,page=19]{tkrAlignNew}
  \includegraphics[width=0.45\textwidth,page=20]{tkrAlignNew}
  \includegraphics[width=0.45\textwidth,page=21]{tkrAlignNew}
  \includegraphics[width=0.45\textwidth,page=22]{tkrAlignNew}
  \includegraphics[width=0.45\textwidth,page=23]{tkrAlignNew}
  \includegraphics[width=0.45\textwidth,page=24]{tkrAlignNew}
  \caption{Alignment of the Silicon planes in the LAT reference system: offset along the x, y, z directions (top left, right and middle left) and rotations around the same axes (middle right, bottom left and right).}
  \label{fig:tkralignment}
\end{figure}

%\begin{figure}[htbp]
%  \centering
%  \includegraphics[width=\textwidth]{tkrAlignment}
%  \caption{Alignment of the Silicon planes in the LAT reference system.\FIXME{procure a real, updated figure}}
%  \label{fig:tkralignment}
%\end{figure}


